IoTFlowGenerator: Crafting Synthetic IoT Device Traffic Flows for Cyber Deception

Over the years, honeypots emerged as an important security tool to understand attacker intent and deceive attackers to spend time and resources. Recently, honeypots are being deployed for Internet of things (IoT) devices to lure attackers, and learn their behavior. However, most of the existing IoT honeypots, even the high interaction ones, are easily detected by an attacker who can observe honeypot traffic due to lack of real network traffic originating from the honeypot. This implies that, to build better honeypots and enhance cyber deception capabilities, IoT honeypots need to generate realistic network traffic flows. To achieve this goal, we propose a novel deep learning based approach for generating traffic flows that mimic real network traffic due to user and IoT device interactions. A key technical challenge that our approach overcomes is scarcity of device-specific IoT traffic data to effectively train a generator. We address this challenge by leveraging a core generative adversarial learning algorithm for sequences along with domain specific knowledge common to IoT devices. Through an extensive experimental evaluation with 18 IoT devices, we demonstrate that the proposed synthetic IoT traffic generation tool significantly outperforms state of the art sequence and packet generators in remaining indistinguishable from real traffic even to an adaptive attacker.

==> original-related-work.tex <==
\section{Related Work} 
\label{sec:related}
%MK: We need related work section.
Our work touches upon multiple different research topics. We discuss the related work in those research areas. 
\subsection{Cyber Deception}
%MK: I like this saying and moving it into the intro.
%Deception has been prevalent throughout history, especially in warfare. As Sun Tzu once wrote in the Art of War\cite{tzu_2005}, "All warfare is based on deception. Hence, when able to attack, we must seem unable; when using our forces, we must seem inactive; when we are near, we must make the enemy believe we are far away; when far away, we must make him believe we are near.” 

In his dissertation, Almeshekah~\cite{almeshekah} gives a definition of deception as a "misperception that is intentionally induced by others". This definition is further explored in \cite{almeshekah2} to describe deception as consisting of two elements: simulation and dissimulation. The purpose of simulation is to represent false information as being true. This work~\cite{almeshekah2} provides three types of actions that can accomplish this act: mimicking, inventing, and decoying. Mimicking mechanisms has the deceiver portray the false information so that it appears to be the truth. Inventing mechanisms create entirely new information that appears to be truthful. Decoying mechanisms attract the adversaries' attention away from the truth. The goal of dissimulation is to hide the truth. In also provide three types of actions that can accomplish dissimulation: masking, repackaging, and dazzling. Masking mechanisms make the truth unable to be detected. Repackaging mechanisms make the truth appear to be something else. Dazzling mechanisms make the truth difficult to be distinguished from false information. We assume these definitions throughout the rest of the paper. Given this definitions, our work can be considered of "inventing" IoT network traffic to create much better decoys that can deceive an attacker.

\subsection{Honeypots}
The number of devices connected to computer networks is growing quickly. This has given rise to an increase in the number of network-based attacks. To protect information systems and related users it is of critical importance to collect accurate, concise, and high-quality information about malicious activities \cite{yegneswaran}. Relying only upon conventional lines of defence such as dynamic firewalls and Intrusion Detection Systems alone does not provide a comprehensive coverage on detecting novel and emerging patterns of attacks \cite{10.1145/2716260}. Honeypots are decoy
computer resources whose value lies in being attacked, probed or compromised \cite{1193207}. They are tools to help spot zero-day attacks and give insights on attackers actions and motivation. \par

A widely used classification of honeypots is based upon the characteristics of interaction \cite{10.1145/1233341.1233399}. We can consider the level of interaction as follows: 1) Low Interaction Honeypots, 2) Medium Interaction Honeypots 3) High Interaction Honeypots.
%\begin{description}
%  \item[$\bullet$ Low Interaction Honeypots]
%  \item[$\bullet$ Medium Interaction Honeypots]
%  \item[$\bullet$ High Interaction Honeypots]
%\end{description}

%MK: I think these paragraphs are very good. I will keep them in a file but we can shorten this discussion. 
\paragraph{A low interaction honeypot} has a limited set of services such as Telnet, SSH and FTP and generally, does not provide access to the operating system to the attacker since this type of honeypot does not have any operating system installed. Low interaction honeypots produce minimal or canned responses in order to allow protocol handshakes. As the availability of information is limited, low interaction honeypots are used mainly for statistical evaluation. These types of honeypots tend to be used in production environments. 

\paragraph{Medium-interaction honeypots}are somewhat more advanced than low interaction honeypots, however they still do not provide any access to the operating system. The simulated services are at a higher level of interaction for the attacker. Medium interaction honeypots produce reasonable replies with the aim to trigger followup attacks. To be a more attractive target, medium interaction honeypots also emulate more services than low interaction honeypots. Because of the lack of access to the operating system, and reduced interaction, low interaction and medium interaction honeypots both have slim chances of being compromised. 

\paragraph{High-interaction honeypots} are the most advanced honeypots. They are the most difficult to implement, deploy and maintain, as they provide to the attacker a real unrestricted operating system environment. Furthermore, a huge set of services is available. High interaction honeypots generally collect the greatest amount of information possible, including complete attack logs, traversing of file trees, data access logs, executed byte codes etc. Because of the complexity, high interaction honeypots log analysis is usually done by networks forensics experts and is less frequently automated. Higher interaction honeypots tend to used for research. Gradually, many different flavors of honeypots were created which were difficult to divide into specific categories, so it became common to only distinguish between low and high interaction honeypots \cite{spitzner_2004}. Anything that is a port listener or emulates is considered low interaction, while anything that provides real services and applications is considered high interaction.

We can also consider the direction of the interaction \cite{honeyc}.

\begin{description}
  \item[$\bullet$ Server Honeypots]
  \item[$\bullet$ Client Honeypots]
\end{description}

Finally, we can also consider the physicality of the honeypots \cite{virtualhoneypot}

\begin{description}
  \item[$\bullet$ Physical Honeypots]
  \item[$\bullet$ Virtual Honeypots]
\end{description}

Server Honeypots wait for attackers to initiate the communication, while client honeypots actively search for potential malicious entities and request an interaction. The most common field of application for client honeypots are web browsers where client honeypots request a homepage and scan for unusual activities. Conventional honeypots are server based. A physical honeypot is a real machine on the network, while a virtual honeypot is simulated or virtualized by a host machine that forwards the network traffic to the virtual honeypot. Multiple virtual honeypots can be simulated on a single host.

\subsection{Internet of Things}
The Internet is quickly evolving and creating various connectivity methodologies. The Internet of Things (IoT) is one of those methodologies which transform current Internet communication to Machine-to-Machine (M2M) basis and can connect ubiquitous devices and facilities with various networks to provide efficient and secure services for all applications anytime and anywhere \cite{iotathreya}. As the number of IoT devices rises, the need to protect these devices also becomes more critical. A study \cite{kaspersky} was conducted in 2017, based on data collected by Kaspersky labs IoT honeypot, that showed about half of malware samples collected are detected in IoT devices, with an increaasing number each year. In the last five years, the number of malwares detected in IoT devices has increased from 46 in 2013 to 7242 in 2017. Below we explore the common architecture of IoT.
\subsubsection{Architecture}
The typical architecture of IoT is divided into three layers \cite{7412116}: 1) application layer; 2) network layer; and 3) perception layer. \par

The perception layer, also known as the sensor layer is the bottom layer in the architecture. The perception layer is the physical layer and interacts with sensors and actuators to acquire information about the environment. Its main objectives are to connect things to the IoT network, and to measure, collect, and process the state information for these things via deployed smart devices, propagating the processed information into upper layers \cite{10.1016/j.comnet.2012.07.010}. This layer mostly consists of sensors and RFIDs, and due to their limited storage capacity, power consumption, and computation capability make them susceptible to many kinds of threats. The confidentiality of this layer can easily be compromised by Replay Attack \cite{7503493} where an intruder can provide a false response on behalf of the destination node to get access to the trusted properties of the source-sensing device. In a timing attack, an attacker can obtain the secret and shared key information by analyzing the encryption algorithm, and predict how much time is needed to get all possible secret keys and use each key to decrypt the encrypted data packets. An attacker can also undermine the integrity of the data in this layer by sending malicious data. This can also lead to a denial of service attack, by consuming the energy of the nodes in the system. The above listed security issues at perception layer can be addressed by using encryption, authentication (to verify true identity of a sender) and access control \cite{7503493}.

The network layer of IoT serves the function of data routing and transmission to various IoT hubs and devices on the Internet. In this layer, cloud computing platforms, Internet gateways, switching, and routing devices etc. operate by using some technologies such as WiFi, LTE, Bluetooth, 3G, Zigbee etc. The network gateways serve as the arbiter between different IoT nodes by aggregating, filtering, and transmitting data to and from different sensors \cite{6996632}. As mentioned previously, the network layer of IoT is susceptible to Denial of Service (DoS) attacks. Aside from the DoS attacks, the adversary can also attack the confidentiality and privacy at network layer by traffic analysis, eavesdropping, and passive monitoring \cite {6970594}.

The application layer defines all applications that use the IoT technology or in which IoT has deployed. The application layer guarantees the authenticity, integrity, and confidentiality of the data. At this layer, the purpose of IoT or the creation of a smart environment is achieved. Since the IoT does not have universal standards that govern the interaction of applications, there are many issues related to application security. Different applications have various authentication mechanisms, which makes integrating them difficult to ensure data privacy and authenticity.

